A Probabilistic Formulation of Unsupervised Text Style Transfer

We present a deep generative model for unsupervised text style transfer that unifies previously proposed non-generative techniques. Our probabilistic approach models non-parallel data from two domains as a partially observed parallel corpus. By hypothesizing a parallel latent sequence that generates each observed sequence, our model learns to transform sequences from one domain to another in a completely unsupervised fashion. In contrast with traditional generative sequence models (e.g. the HMM), our model makes few assumptions about the data it generates: it uses a recurrent language model as a prior and an encoder-decoder as a transduction distribution. While computation of marginal data likelihood is intractable in this model class, we show that amortized variational inference admits a practical surrogate. Further, by drawing connections between our variational objective and other recent unsupervised style transfer and machine translation techniques, we show how our probabilistic view can unify some known non-generative objectives such as backtranslation and adversarial loss. Finally, we demonstrate the effectiveness of our method on a wide range of unsupervised style transfer tasks, including sentiment transfer, formality transfer, word decipherment, author imitation, and related language translation. Across all style transfer tasks, our approach yields substantial gains over state-of-the-art non-generative baselines, including the state-of-the-art unsupervised machine translation techniques that our approach generalizes. Further, we conduct experiments on a standard unsupervised machine translation task and find that our unified approach matches the current state-of-the-art.

==> ack.tex <==
\paragraph{Acknowledgements:} This work was supported in part by the DARPA GAILA program under award HR00111990063, and a gift from the Tang Family Foundation.

==> experiment.tex <==
\section{\label{sec:experiment}Experiments}
We test our model on five sequence transduction tasks: sentiment transfer, word substitution decipherment, formality transfer, author imitation, and related language translation. We select these tasks as relatively easy test beds for unsupervised methods. For example, sentiment/formality/author transfer tasks share vocabulary across domains, word substitution decipherment has one-to-one correspondence between the vocabularies of the source and target domains, and related language translation assumes grammar or typology similarity between the language pairs. For more difficult tasks like unsupervised machine translation, carefully pre-trained embeddings or model initialization from external knowledge are necessary to obtain descent performance~\citep{lample2018phrase,Lample2019CrosslingualLM,artetxe2019effective}. In this paper, however, we focus on evaluations that do not require external knowledge. 

We compare with the unsupervised machine translation model (UNMT) which recently demonstrates state-of-the-art performance on text rewriting tasks such as sentiment transfer and gender transfer~\citep{lample2018multipleattribute}.\footnote{Note that the model they used is slightly different from the original UNMT model~\citep{lample2018phrase} on some details like adding a pooling layer after attention to achieve better performance. Since the authors could not release the code due to legal issues (at the time we run experiments in this paper), we re-implement their model in our codebase for fair comparison. We verify that our re-implementation is able to achieve competitive performance compared with the original paper.} To validate the effect of the negative entropy term in the KL loss term Eq.~\ref{eq:kl}, we remove it and train the model with a back-translation loss plus a language model negative log likelihood loss (which we denote as BT+NLL) as an ablation baseline. For each task, we also include strong baseline numbers from related work if available. To ensure a totally unsupervised setting, we never use parallel data for selecting the best validation model. Complete model configurations and hyperparameters can be found in Appendix~\ref{app:implementation}. 

% \gn{It would be really nice to at least have a few qualitative examples. Maybe on the tasks where we do best such as related language translation?}

% \gn{It seems like a waste of space to scatter the results over so many tables and discuss them separately in different sections. I'm not sure the best way to do things, but there must be a better way?}

\begin{wraptable}{r}{0.4\textwidth}
\vspace{-1cm}
\begin{center}
    \captionof{table}{\label{tab:cipher_results}Results on decipherment.}
    \begin{tabular}{lr}
    \toprule
    %\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{BLEU}} & \multirow{2}{*}{\textbf{ACC.}} & \multicolumn{2}{c}{\textbf{PPL.}} \\
    \textbf{Model} & \textbf{BLEU}  \\
    \midrule
    \citet{shen2017style} &  50.8  \\
    \citet{yang2018unsupervised} & 49.3  \\
    \midrule
    UNMT &  76.4 \\
    BT+NLL & 78.0  \\
    Ours &  \bf 78.4 \\
    %\midrule
    \bottomrule
    \end{tabular}
    \vspace{-13pt}
\end{center}
\end{wraptable}
\subsection{Word Substitution Decipherment}
\label{sec:exp-decipher}
The word decipherment task aims to uncover the plain text that lies behind an enciphered corpus. For substitution ciphers, each word in the vocabulary is mapped to a unique token in the cipher dictionary. This task has been widely used in prior work~\citep{decipher,shen2017style,yang2018unsupervised}. In our formulation, our model is presented with English plaintext sentences and a ciphertext corpus without parallel data. We use the data in~\citep{yang2018unsupervised} which provides 200K sentences from each domain. While previous work~\citep{shen2017style,yang2018unsupervised} controls the difficulty of this task by varying the percentage of words that are ciphered, we directly evaluate on the most difficult version of this task -- 100\% of the words are enciphered (i.e.\ no vocabulary sharing in the two domains). We select the model with the best unsupervised reconstruction loss, and evaluate with BLEU score on the test set which contains 100K parallel sentences.

% We can control the percentage of words to be replaced by their cipher tokens as a way to control the difficulty of decipherment. Here we directly use the most difficult setting of the task, that is, replacing all the words with their cipher tokens. task commonly used in previous work

% Following the setup in prior work~\citep{yang2018unsupervised,shen2017style}, we sample 200K sentences from the Yelp dataset as sequences in domain X. We then create the domain Y sequences by sampling another 200K sentences and replacing all the words by their corresponding cipher tokens.

% \paragraph{Baselines.} We compare our model with several strong baselines: 1) \citep{lample2018multipleattribute}: this is the state-of-the-art model on unsupervised multiple-attribute text style transfer. The model combines back-translation with an denoising autoencoder; 2) \citep{yang2018unsupervised}: this is the model that achieves the state-of-the-art performance on the Yelp dataset. It uses language models as discriminators to encourage learning style-independent representations.

% \paragraph{Our model.} We consider two different settings of our model: 1) Full: the full model using language model KL divergence as the prior; 2) Dual: the same model except we use the \cw{Not super sure about the setting here, maybe we should explain more somewhere else and i can just refer here}  

\vspace{-5pt}
\paragraph{Results:} The results are shown in Table~\ref{tab:cipher_results}. We find that the UNMT baseline, which uses a sequence-to-sequence model with attention, already achieves strong results on this task, improving over the previous state-of-the-art result by over 25 BLEU points. The performance improvements of UNMT indicate that flexible and powerful architectures are crucial~(prior methods generally do not have attention mechanism). Compared to the already strong UNMT baseline, our model still achieves a 2 BLEU point improvement, reaching 78.4 BLEU, while BT+NLL also obtains competitive results. This indicates the benefit from a language model. We also conducted an ablation experiment, where we remove parameter sharing~(as explained in Section \ref{sec:learning}) between two directions of transduction distributions, and optimize two encoder-decoder instead. We found that the model only obtained an extremely low BLEU score and failed to generate any meaningful outputs. Therefore, we do not consider this baseline for the rest of the datasets.

% \subsection{Evaluation}
% For the unsupervised sequence transduction task, we want to \textit{preserve the content} of the source domain sequence, while rewriting it into the attribute of the target domain. Although the automatic evaluation metrics for the task is still an open research problem, we follow some standard practice in prior works on text style transfer\cite{lample2017unsupervised,yang2018unsupervised}. Specifically, we use three different categories of automatic metrics for evaluation.
% \paragraph{BLEU score.} We measure the content preservation using BLEU score\cite{}, a commonly used metric in Machine Translation that essentially compares the $n$-gram statistics between the model output and the reference. Following \cite{lample2018multipleattribute}, we measure both 1) BLEU$_s$~(self BLEU): the BLEU score between the model output and its input; 2) BLEU$_r$~(reference BLEU): the BLEU score between the model output and the reference, if the reference document is provided.

% \paragraph{Classification Accuracy.} We use classification accuracy to measure the extent to which our model is able to successfully transduce the source sequence into the target domain. 

% \paragraph{Perplexity.} We additionally measure the perplexity of the model output using language models trained on the target domains. For the rest of the section, we denote the two domains for each task as $X$ and $Y$, and report the perplexity of each domain. This metric indicates the quality of the generated sentences. In general lower perplexity indicates a better output quality. However, it is important to note that sometimes the model output can achieve abnormally low perplexity if most of its contents are very simple and short sentences, such as ``I like this place''. Ideally, good quality sentences from a given domain should have perplexity that is close to the language model's perplexity on the test set of that domain. In the following sections, we will point out the cases when the output perplexity is even much lower than the perplexity of the test set.


\subsection{Sentiment Transfer}
Sentiment transfer is a task of paraphrasing a sentence with a different sentiment while preserving the original content. Evaluation of sentiment transfer task is difficult and is still an open research problem~\citep{Mir2019EvaluatingST}. Specifically, we need to evaluate the output from three aspects: attribute control, content preservation, and fluency. A successful system needs to perform well with respect to all of these three aspects. 
%Even with parallel test corpus, the evaluation is still challenging. Because the parallel sentences of different sentiments share a lot of content words, simple self-copy could obtain a descent reference BLEU score while completely fail in successful transfer. 
We follow prior work in terms of evaluation by using three metrics~\citep{yang2018unsupervised,lample2018multipleattribute}: classification accuracy, self-BLEU (BLEU of the output with the original sentence as the reference), and perplexity (PPL) to evaluate the three axes. We pretrain a convolutional classifier~\citep{kim2014convolutional} to assess classification accuracy, and LSTM language models on each domain to compute perplexity.\footnote{In our model, the pretrained LSTM language models are also used as the prior.} For reference, the language models obtain perplexity 31.97 and 21.87 on the positive and negative test sets, respectively.

We use the Yelp reviews dataset collected by~\citet{shen2017style} which contains 250K negative sentences and 380K positive sentences. Besides the test set from the dataset itself, we also use a small test set that has 1000 human-annotated parallel sentences introduced in~\citet{li2018delete}. We denote the positive sentiment as domain $\gD_1$ and the negative sentiment as domain $\gD_2$. We denote self-BLEU score as BLEU$_s$ and reference BLEU score on the 1000 sentences as BLEU$_r$. 
\vspace{-5pt}
\paragraph{Interpreting Evaluation:}We use a combination of different metrics, measuring sometimes conflicting aspects of the model output. For example, models with higher classification accuracy tend to have lower BLEU score, because the output substantially changes the input content to successfully control sentiment. In general, a model can make tradeoffs among these metrics by using different hyperparameters. To account for this tradeoff for better evaluation of different models, we run 3 sets of experiments for each model with different hyperparameters to obtain 3 data points on the classification-BLEU curve, and report the one with the median accuracy\footnote{We find that the one with median accuracy usually represents the best balance between attribute control and BLEU. In contrast, a high accuracy with low BLEU score or a low accuracy with high BLEU score are generally from trivial outputs, which indicates complete failure of the model.}, and we include the full results in Appendix \ref{app:full_table}. We also emphasize that PPL should be evaluated together with reference to the PPL of the test set from the target domain. This is because extremely low PPL could indicate that the generated sentences are overly trivial, such as all very short sentences. 
%While perfect transduction should have similar PPL to the numbers on the test corpus from the target domain.

% \paragraph{Baselines.} Besides the baselines by \cite{yang2018unsupervised} and \cite{lample2018multipleattribute}, we also compare with a few other prior works on this dataset: 1) \citep{shen2017style}: it uses 3 discriminators to align the latent variables and decoder hidden states; 2) \citep{hu2017toward}: this method uses a pretrained classifier combined with a VAE. 
\vspace{-5pt}
\paragraph{Results:} The results are shown in Table~\ref{tab:yelp_results}. BT+NLL obtains an unreasonably low PPL, which is much lower than the PPL of the test corpus in the target domain. After a close examination of the output, we find that it contains many repeated and overly simple outputs. For example, the system generates many examples of ``I love this place'' when transferring negative to positive sentiment (see Appendix~\ref{app:sentiment-eg} for examples). It is not surprising that such a trivial output has low perplexity, high accuracy, and low BLEU score. On the other hand, our system obtains reasonably competitive PPL, which indicates the effectiveness of the additional entropy regularizer in Eq.~\ref{eq:kl} that is the byproduct of our probabilistic formulation. Also, our approach achieves the highest accuracy and higher BLEU score than the UNMT baseline.~\citet{hu2017toward} obtains higher self-BLEU score than our method, but its output is less fluent~(with high PPL), which is also observed in previous work~\citep{yang2018unsupervised,lample2018multipleattribute}. 
%\resizebox{!}{2cm}{
%\begin{wraptable}{l}{0.6\textwidth}
\begin{center}
    \vspace{-0.2cm}
    \captionof{table}{\label{tab:yelp_results}Results on the sentiment transfer task.}
    \begin{tabular}{lrrrrr}
    \toprule
    %\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{BLEU}} & \multirow{2}{*}{\textbf{ACC.}} & \multicolumn{2}{c}{\textbf{PPL.}} \\
    \textbf{Model} & \textbf{Acc.} & \textbf{BLEU$_r$} & \textbf{BLEU$_s$}  & \textbf{PPL}$_{\gD_1}$ & \textbf{PPL}$_{\gD_2}$ \\
    \midrule
    \citet{shen2017style} & 79.50 & 6.80 & 12.40  & 50.40 & 52.70 \\
    \citet{hu2017toward}  & 87.70 & - & \textbf{65.60}  & 115.60 & 239.80 \\
    \citet{yang2018unsupervised}  & 83.30 & 13.40 & 38.60 & 30.30 & 42.10 \\
    \midrule
    UNMT & 87.17   & 16.99 & 44.88 & 26.53 & 35.72 \\
    BT+NLL  & \textbf{88.36} & 12.36 & 31.48 & 8.75 & 12.82 \\
    Ours  & 87.90 & \textbf{18.67} & 48.38 & 27.75 & 35.61 \\
    %\midrule
    \bottomrule
    \end{tabular}
    % \vspace{0.2cm}
    \end{center}
%\end{wraptable}
%}
\subsection{Formality Transfer}
%\begin{table}[h]
\begin{wraptable}{r}{0.55\textwidth}
\vspace{-1.5cm}
\begin{center}
    \captionof{table}{\label{tab:from_results}Results on the formality transfer task.}
    \begin{tabular}{lrrrr}
    \toprule
    %\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{BLEU}} & \multirow{2}{*}{\textbf{ACC.}} & \multicolumn{2}{c}{\textbf{PPL.}} \\
    \textbf{Model}  & \textbf{Acc.} & \textbf{BLEU$_r$} & \textbf{PPL}$_{\gD_1}$ & \textbf{PPL}$_{\gD_2}$ \\
    \midrule
    UNMT & 78.06 & 16.11 & 26.70 & 10.38 \\
    BT+NLL  & \bf 82.43 & 8.57 & 6.57 & 8.21 \\
    Ours  & 80.46 & \textbf{18.54} & 22.65 & 17.23 \\
    %\midrule
    \bottomrule
    \end{tabular}
    %\vspace{0.2cm}
\end{center}
\end{wraptable}
%\end{table}
Next, we consider a harder task of modifying the formality of a sequence. We use the GYAFC dataset~\citep{rao2018dear}, which contains formal and informal sentences from two different domains. In this paper, we use the Entertainment and Music domain, which has about 52K training sentences, 5K development sentences, and 2.5K 
test sentences. This dataset actually contains parallel data between formal and informal sentences, but we treat the dataset as a nonparallel corpus. 
% We use Moses tokenizer to preprocess the whole dataset. 
We follow the evaluation of sentiment transfer task and test models on three axes. Since the whole test set is a parallel corpus, we only compute reference BLEU and ignore self-BLEU. We use $\gD_1$ to denote formal text, and $\gD_2$ to denote informal text. The perplexity of the test set from domain $\gD_1$ and $\gD_2$ is 71.30 and 135.50, respectively. 
\vspace{-10pt}
\paragraph{Results:} We list the results with median accuracy of different methods in Table \ref{tab:from_results}, and the full results of all three runs of each method can be found in Appendix \ref{app:full_table}.  We can see that BT+NLL again has abnormally low perplexity, along with high accuracy and extremely low BLEU, indicating this method fails to generate meaningful output. Our method outperforms UNMT in both accuracy and BLEU score. The PPL of both UNMT and our model are much lower than the test PPL, which indicates both of the methods might have issue of generating complex output as in the reference. 

%\tberg{Maybe word decipherment first? Treat it kind of like an analysis task where we show that the model can recover sequence structure when we know the mapping is 1-1. Then go on to harder, noisier tasks} 

\subsection{Author Imitation}
\begin{wraptable}{r}{0.55\textwidth}
\vspace{-1cm}
\begin{center}
%\begin{table}[h]
%    \centering
    \captionof{table}{\label{tab:shake_results}Results on the author imitation task.}
    \begin{tabular}{lrrrrr}
    \toprule
    %\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{BLEU}} & \multirow{2}{*}{\textbf{ACC.}} & \multicolumn{2}{c}{\textbf{PPL.}} \\
    \textbf{Model}  & \textbf{Acc.} & \textbf{BLEU$_r$} & \textbf{PPL}$_{\gD_1}$ & \textbf{PPL}$_{\gD_2}$ \\
    \midrule
    UNMT & 80.23  & 7.13 & 40.11 & 39.38 \\
    BT+NLL & 76.98 & 10.80 & 61.70 & 65.51 \\
    Ours & \textbf{81.43}  & \textbf{10.81} & 49.62 & 44.86 \\
    %\midrule
    \bottomrule
    \end{tabular}
    \vspace{-13pt}
%\end{table}
\end{center}
\end{wraptable}

For the author imitation task, we want to test the model's ability of paraphrasing a sentence according to certain author styles. The dataset we use is a collection of Shakespeare's plays translated line by line into modern English. It was collected by \cite{shakespeare_data}\footnote{We downloaded the data from \url{https://github.com/tokestermw/tensorflow-shakespeare}} and used in some prior work on writer style transfer~\citep{shakespearizing_copy_model}. This is a parallel corpus and thus we follow the setting in the formality transfer task. We use $\gD_1$ to denote modern English, and $\gD_2$ to denote Shakespeare-style English. The perplexity of the test set from domain $\gD_1$ and $\gD_2$ is 132.95 and 85.25, respectively.
\vspace{-5pt}
\paragraph{Results:} The main results of the dataset can be found in Table \ref{tab:shake_results}, and the full result table is in Appendix \ref{app:full_table}. Our model again outperforms the strong UNMT baseline. Our method has slightly higher perplexity than the baseline. However, it is important to note here that again the perplexity of all methods is lower than the test set from the target domain, so lower perplexity probably does not correlate well with better sentence quality.  

\subsection{Related Language Translation}
\begin{wraptable}{r}{0.45\textwidth}
\vspace{-1cm}
\begin{center}
%\begin{table}[h]
%    \centering
    \captionof{table}{\label{tab:trans_results}BLEU-1 scores on related language translation.}
    \begin{tabular}{lrr}
    \toprule
    %\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{BLEU}} & \multirow{2}{*}{\textbf{ACC.}} & \multicolumn{2}{c}{\textbf{PPL.}} \\
    \textbf{Model} & \textbf{sr-bs} & \textbf{bs-sr} \\
    \midrule
    \cite{yang2018unsupervised} & 31.00 & 33.40  \\
    \midrule
    UNMT & 31.40 & 33.40  \\
    BT+NLL & 29.60 & 31.40  \\
    Ours &  \textbf{36.20} & \textbf{38.30} \\
    %\midrule
    \bottomrule
    \end{tabular}
    \vspace{-13pt}
%\end{table}
\end{center}
\end{wraptable}
Finally, we test our method on a challenging related language translation task~\citep{decipher_language,yang2018unsupervised}. This task is a natural test bed for unsupervised sequence transduction, because the goal is to preserve the meaning of the source sentence while rewriting it into the target language. For our experiments, we choose Bosnian~(bs) and Serbian~(sr) as the related language pairs. We follow~\citet{yang2018unsupervised} to report BLEU-1 score on this task since BLEU-4 score is close to zero.
\vspace{-10pt}
\paragraph{Results:} For translation in both directions, UNMT achieves comparable performance with the state-of-the-art baseline method in \cite{yang2018unsupervised}, while BT+NLL is lower than the baseline. Our method, however, brings a large 5 BLEU gain for translations in both directions. 


==> introduction.tex <==
\section{Introduction}
\label{sec:intro}
Text sequence transduction systems focus on converting a given text sequence from one domain to another. These techniques can be applied to a wide range of natural language processing applications such as machine translation~\citep{bahdanau2014neural}, summarization~\citep{rush2015neural}, and dialogue response generation~\citep{zhao2017learning}.
% \gn{Need citations. Also, sentiment transfer and style transfer are not typical (supervised) sequence transduction tasks, so maybe it'd be a better idea to lead off with something like MT, summarization, and dialog response generation? Then after the following sentence where you note the paucity of data in some situations, you could say that reliance on supervised data prevents application to these tasks.}. 
In many cases, however, parallel corpora for the task at hand is scarce -- for example, it is difficult to find parallel translations for low-resource languages. Therefore, \textit{unsupervised} sequence transduction methods that require only non-parallel data are appealing and have been receiving growing attention~\citep{bannard2005paraphrasing,ravi2011deciphering,mizukami2015linguistic,shen2017style,lample2018phrase,lample2018multipleattribute}.

Recent work on unsupervised text transduction mostly employs non-probabilistic modeling approaches. For example,~\citet{shen2017style} and \citet{yang2018unsupervised} design adversarial discriminators to shape their unsupervised objective -- an approach that can be effective, but often introduces training instability. Another line of work focuses on directly designing unsupervised training objectives by incorporating intuitive loss terms (e.g. backtranslation loss), and demonstrates state-of-the-art performance on unsupervised machine translation~\citep{lample2018phrase,artetxe2019effective} and style transfer~\citep{lample2018multipleattribute}. While these approaches can also be effective, the space of possible unsupervised objectives is extremely large and the underlying modeling assumptions defined by each objective can only be reasoned about indirectly. As a result, the process of designing such systems is often heuristic. 

In contrast, probabilistic models (e.g.\ the noisy channel model~\citep{shannon1948mathematical}) define their assumptions about data more explicitly and allow us to reason directly about these assumptions during system design. Further, the corresponding unsupervised objectives are determined naturally by the principles of probabilistic inference, reducing the need for empirical search directly in the space of possible objectives. That said, classical probabilistic models for unsupervised sequence transduction (e.g. the HMM or semi-HMM) typically enforce overly strong independence assumptions about data to make exact inference tractable~\citep{knight2006unsupervised,ravi2011deciphering,decipher_language}. This has restricted their development and caused their performance to lag behind unsupervised neural objectives on complex tasks. Luckily, in recent years, powerful variational approximation techniques have made it more practical to train probabilistic models without strong independence assumptions~\citep{miao2016language,yin2018structvae}. Inspired by this, we take a new approach to unsupervised sequence transduction. 

We directly define a generative probabilistic model that treats a non-parallel corpus in two domains as partially observed parallel corpus – reflecting our intuitive assumptions about the data generating process. Our model makes few independence assumptions and its true posterior is intractable. However, we show that by using amortized variational inference~\citep{kingma2013auto}, a principled probabilistic technique, a natural unsupervised objective falls out of our modeling approach that has many connections with past work, yet is different from all past work in specific ways. In experiments across five unsupervised text transductions tasks, we find that the natural objective of our model actually outperforms all manually defined unsupervised objectives from past work, supporting the notion that probabilistic principles can be a useful guide even in deep neural systems.

% However, we argue that which shen2017style, Recently~\citet{yu2016neural} try to extend the decoder in noisy channel model with flexible neural network, but still Classically a popular framework to perform unsupervised text transdution is to maximize data distribution through a probabilistic generative model (e.g.\ the well-known noisy channel model~\citep{shannon1948mathematical}, which has facilitated successful applications to word decipherment~\citep{knight2006unsupervised} and translation~\citep{ravi2011deciphering,decipher_language}. While these methods provide principled ways to learn the transduction distribution, they typically enforce overly strong simplifying assumptions about data to make inference practical. 

% While existing neural methods in this direction are mostly non-probabilistic~\citep{yang2018unsupervised,artetxe2018unsupervised,lample2018phrase,lample2018multipleattribute}, we argue that pro 

% Classific Existing work in this direction relies on heuristic training objectives to achieve competitive performance \gn{What do you classify as ``heuristic''? \citet{shen2017style} and \citet{yang2018unsupervised} seem like reasonably well-defined objectives. Could you clarify?} \tberg{What if we refer to prior work as non-probabilistic? Our arugment, after all, is mainly about the benefits of probabilistic modeling for this task. Prob models are typically more stable than GANs during training. And they come with principled learning and inference technqiues. Prob model takes a lot of the guesswork out of designing unsup objectives. Past work has focused directly on designing objectives. In contrast, we focus on designing a model, and the objective is byproduct. Argue that it is easier to reason about modeling assumptions in terms of a model than in terms of a direct objective function. We show that starting with a model, and letting its assumption define the objective, actually leads to a better objective than past work! Finally, we don't have to call past work "heuristic" which is a little strong -- but we could argue that the process of designing GANs and directly defined unsupervised objectives is more heuristic in nature than designing prob models. I think most would agree with that? }. For example, backtranslation loss~\citep{sennrich2016improving} is believed to play a critical role in unsupervised machine translation methods as a data augmentation technique~\citep{artetxe2018unsupervised,lample2018unsupervised,lample2018phrase}, whereas, on text style transfer tasks, a discriminator is often applied to the output side to control its attributes (e.g. sentiment~\citep{hu2017toward,yang2018unsupervised}).~\citet{artetxe2019effective} explore an additional language model loss for the text generation side, which can be explained as a reward function from the perspective of reinforcement learning~\citep{he2016dual}. 

% \gn{Given the previous paragraph it's not clear why this is a good idea worth pursuing (and accepting to NeurIPS). Why does this solve problems of previous methods, or what benefits does it bring?} \tberg{Agree with Graham -- need to emphasize WHY prob model. I think the stuff I mentioned in above comment would be useful here. Overall I see the contribution like this: (1) It is reasonable to think that designing systems in terms of probabilistic models has benefits over directly defining unsupervised objectives. The space of possible unsupervised objectives is huge, and the underlying assumptions and learning signal each objective produces must be reasoned about indirectly -- the process of designing such systems is often heuristic. In contrast, probabilistic models define their assumptions about data explicitly. We can reason directly about these assumptions during system design, and the corresponding unsupervised objectives are determined naturally by the principles of probabilistic inference. However, since exact inference is often intractable -- classical models typically enforce overly strong simplying assumptions about data to make inference practical. 
% (2) Luckily, in recent years, powerful variational approximation technqiues have made it more practical to use probalisitic models without strong assumptions. Inspired by this, we take a new approach to unsupervised sequence transduction. We directly define a generative probablistic model that treats a non-parallel corpus as partially observed parallel corpus -- reflecting our intuitive assumptions about the data generating process. Our model makes few assumptions and its true posterior is intractable.
% (3) However, we show that by using amortized variational inference, a principled probalisitic technqiue, a natural unsupervised objective falls out of our modeling approach that has many connections with past work, yet is different from all past work in specific ways. We find that the natural objective of our model actually outperforms ALL manually defined unsupervised objectives from past work, supporting the notion that probabilistic principles can be a useful guide even in deep neural systems. 
% }
% In this paper we propose a probabilistic generative model to perform unsupervised text sequence transduction. In our method, a non-parallel collection of sentences from two domains is modeled as a partially observed parallel corpus -- given a data sample from one domain, its corresponding sentence in another domain is treated as an unobserved latent sequence. Specifically, a recurrent language model is pre-trained as the prior distribution for the latent sequence, and the generator is defined with an encoder-decoder architecture. Due to the intractable marginal data likelihood in this deep latent sequence model, we utilize amortized variational inference~\citep{kingma2013auto} to optimize the evidence lower bound (ELBO) as a surrogate. In contrast with deep latent variable models where latent variables are continuous vectors, the inference network in our model consists of an encoder-decoder structure, similar to the channel model \tberg{and, critically, we show that sharing parameters ... necessary} . Some previous methods have tried modeling compressed sentences~\citep{miao2016language} or structured queries~\citep{yin2018structvae} as latent sequence variables, our approach differs in that we focus on the completely unsupervised setting while they mainly aim to augment data in a semi-supervised fashion \tberg{mention parameter sharing as something difference from structVAE}. 
% % Traditional sequence to sequence generative models (e.g.\ the noisy channel model) for unsupervised sequence transduction~\citep{knight2006unsupervised} follows the well-known noisy-channel framework, our model makes few assumptions about the transduction distribution and can 

% \gn{This paragraph feels a bit scattered and long. I feel maybe just the first three sentences should be OK. Some of the remainder of the paragraph can be moved to the next paragraph.}
% We further show that some known effective heuristics from past unsupervised sequence transduction work can be connected with our probabilistic framework (Section~\ref{}): the backtranslation loss naturally appears as the reconstruction term in ELBO. Also,~\citet{yang2018unsupervised} uses a language model as the discriminator and imposes an adversarial loss on the output side,~\citet{artetxe2019effective} adds a pretrained language model to compute the reward, these losses are part of the KL divergence term in ELBO, in experiments we demonstrate that the KL loss in ELBO is practically superior to the baseline language model loss. Our unified probabilistic formulation enables us to draw inspiration from standard latent variable models, and potentially offers a more principled way to regularize the sentence transduction posterior via the prior. For example, in addition to language model priors, some specially designed structured distribution such as tree or Markov structures --which are often desirable for clearly-structured latents like SQL queries-- can be defined as the prior to be easily injected as regularization of learning the transduction model.

% Our model is validated on a wide range of unsupervised text transduction tasks including sentiment transfer, formality transfer, word decipherment, shakespearizing modern language, and related language translation. Across all tasks, our approach yields gains over \gnc{competitive}{state-of-the-art} \gn{can we say this?} non-generative baselines.

==> method.tex <==
\section{Unsupervised Text Transduction}
% \gn{Made this a top-level section to separate background and proposed methods.}

We first give a brief overview of the task of text transduction, which aims to transfer a text (typically a single sentence or a short paragraph -- for simplicity we refer to sentences in our model description) from one domain to another while preserving underlying content. For example, informal-formal transfer~\citep{rao2018dear}, the task of transforming the formality style of a paragraph from informal to formal without changing its basic content, is a text transduction task. Other examples include sentiment transfer~\citep{shen2017style}, word decipherment~\citep{knight2006unsupervised}, and machine translation~\citep{bahdanau2014neural}. When parallel examples are available from each domain (i.e. the training data is a bitext consisting of pairs of sentences from each domain) supervised techniques can be used to accomplish text transduction. In this case, the task closely matches that of supervised machine translation and standard model classes (e.g. attentional Seq2Seq~\citep{bahdanau2014neural} and Transformer~\citep{vaswani2017attention}) have proven successful.

% \gn{In the following description, particularly in the modeling part, I got a bit confused by both full corpora and sentences being represented by lowercase bold symbols. Perhaps you could make the corpora $X$ and $Y$ or $\mathcal{X}$ and $\mathcal{Y}$ to make the distinction clear.}

For many domains, however, parallel data is not readily available while non-parallel corpora, one corpus from each domain, can be collected easily. Learning to perform transduction from non-parallel data represents a harder problem and is referred to as \textit{unsupervised} text transduction. The model we propose treats the observed non-parallel text corpus as a partially observed parallel corpus. Thus, we introduce notation for both observed text inputs and those that we will treat as latent variables. Specifically, we let $\xc =\{\x^{(1)}, \x^{(2)},\cdots, \x^{(m)} \}$ represent observed data from domain $\gD_1$, while we let $\yc =\{\y^{(m+1)}, \y^{(m+2)},\cdots, \y^{(n)} \}$ represent observed data from domain $\gD_2$. Corresponding indices represent parallel sentences. Thus, none of the observed sentences share indices. In our model, we introduce latent sentences to complete the parallel corpus. Specifically, $\bar\xc =\{\bx^{(m+1)}, \bx^{(m+2)},\cdots, \bx^{(n)} \}$ represents the set of latent parallel sentences in $\gD_1$, while $\byc =\{\by^{(1)}, \by^{(2)},\cdots, \by^{(m)} \}$ represents the set of latent parallel sentences in $\gD_2$. Then the goal of unsupervised text transduction is to infer these latent variables conditioned the observed non-parallel corpora; that is, to learn $p(\by | \x)$ and $p(\bx | \y)$.

\section{The Deep Latent Sequence Model}

In this section we present the structure of our generative model of bitext, which we refer to as a deep latent sequence model. We then describe approximate learning and inference techniques that enable unsupervised text transduction using this model class.

\subsection{Model Structure}
\begin{figure}[!t]
\centering
     \includegraphics[scale=0.13]{figure/model.png}
     \caption{Graphical representation of the proposed generative models. Shaded circles denote the observed variables and unshaded circles denote the latents. The generator is parameterized as an encoder-decoder architecture and the prior on the latent variable is a pretrained language model.}
    \label{fig:model}
    \vspace{-13pt}
\end{figure}

Directly modeling $p(\by | \x)$ and $p(\bx | \y)$ in the unsupervised setting is difficult because we never directly observe parallel data. Instead, we propose a generative model of the complete data that defines a joint likelihood, $p(\xc, \bxc, \yc, \byc)$. In order to perform text transduction, the unobserved halves can be treated as latent variables: they will be marginalized out during learning and inferred via posterior inference at test time. 

Our model assumes that each observed sentence is generated from an unobserved parallel sentence in the opposite domain, as depicted in Figure 1. Specifically, each sentence $\x^{(i)}$ in domain $\gD_1$ is generated as follows:  First, a latent sentence $\bar\y^{(i)}$ in domain $\gD_2$ is sampled from a prior, $p_{\mathcal{D}_2}(\bar\y^{(i)})$. Then, $\x^{(i)}$ is sampled conditioned on $\bar\y^{(i)}$ from a transduction model, $p(\x^{(i)}|\bar\y^{(i)})$. Similarly, each observed sentence $\y^{(j)}$ in domain $\mathcal{D}_2$ is generated conditioned on a latent sentence, $\bar\x^{(j)}$, in domain $\mathcal{D}_1$ via the opposite transduction model, $p(\y^{(j)}|\bar\x^{(j)})$, and prior, $p_{\mathcal{D}_1}(\bar\x^{(j)})$. We let $\thetaxy$ and $\thetayx$ represent the parameters of the two transduction distributions respectively. We assume the prior distributions are pretrained on the observed data in their respective domains and therefore omit their parameters for simplicity of notation. Together, this gives the following joint likelihood:
% \gn{in the following equation you go from a model that calculates conditional probabilities over single sentences ($p(\y^{(j)}|\bar\x^{(j)})$) to one that calculates probabilities over full corpora ($p(\y|\bar\x)$) without any particular mention of the switch. I'd try to make this clear.}
{\small
\begin{equation}
\label{eq:joint}
p(\xc, \bxc, \yc, \byc; \thetaxy, \thetayx) =  \left(\prod^m_{i = 1}p\big(\x^{(i)}|\by^{(i)}; \thetaxy\big) p_{\gD_2}\big(\by^{(i)}\big) \right) \left(\prod^n_{j = m+1}p\big(\y^{(j)}|\bx^{(j)}; \thetayx\big) p_{\gD_1}\big(\bx^{(j)}\big) \right)
\end{equation}}
The log marginal likelihood of the observed data, which we will approximate during training, can be written as:
\begin{equation}
\label{eq:marginal}
\log p(\xc, \yc; \thetaxy, \thetayx) = \log \sum\nolimits_{\bxc} \sum\nolimits_{\byc} p(\xc, \bxc, \yc, \byc; \thetaxy, \thetayx)
\end{equation}
Note that if the two transduction models share no parameters, the training problems for each observed domain are independent. Critically, we introduce parameter sharing through our variational inference procedure, which we describe in more detail in Section~\ref{sec:learning}.
% where $\thetaxy$ and $\thetayx$ parameterize $p(\x|\by)$ and $p(\y|\bx)$ respectively. In this paper we focus on using a language model pretrained on $\x$ and $\y$ as the prior $\plx$ and $\ply$, respectively. 
\vspace{-5pt}
\paragraph{Architecture: }
Since we would like to be able to model a variety of transduction tasks, we choose a parameterization for our transduction distributions that makes no independence assumptions. Specifically, we employ an encoder-decoder architecture based on the standard attentional Seq2Seq model which has been shown to be successful across various sequence to sequence tasks~\citep{bahdanau2014neural,rush2015neural}. Similarly, our prior distributions for each domain are parameterized as recurrent language models which, again, make no independence assumptions. In contrast, traditional unsupervised generative models typically make strong independence assumptions to enable exact inference (e.g. the HMM makes a Markov assumption on the latent sequence and emissions are one-to-one). Our model is more flexible, but exact inference via dynamic programming will be intractable. We address this problem in the next section.
% However, there is no dynamic program to marginalize over the latent sequence in our model -- unlike an HMM -- since neither prior nor transduction model factors over the latent sequence. Next we will discuss the training method and show our model is still learnable from unsupervised data while being flexible. 

% \tberg{IMPORTANT: We should separate out the parameterization of the model into a separate short sub-section called "Architecture". I'm worried reviewer will miss the sentence about the transduction model being an encoder-decoder -- this is really important because it's what makes our model not just a simple HMM. In the new sub-section, we could also spend a sentence or two talking about why encoder-decoder w/ attention is a powerful model for transduction, but that it is hard to train in an unsupervised setting. Can cite prior work with Enc-dec w / attention here too. Also point out how this parameterization makes our model different than classifical models like HMMs, which, up to the point where we describe the architecture, could be in our model class. You can say that typically unsupervised models have to make strong independence assumptions which restrict their use -- e.g. HMM makes markov and 1-1 assumption, semi-Markov not 1-1 but still Markov. For problems that are mostly 1-1, but not completely this can cause problems. Our model is flexible, and as we show in experiments, still learnable from unsupervised data. In this section, you could actually refer to the individual words $\x_{ij}$ and write out the decoder distribution $p(\x_{i1},$} The generator parameterizes the transduction distribution $\pxy$ or $\pyx$ with an encoder-decoder architecture, which can be instantiated with a normal attentional Seq2Seq model~\citep{bahdanau2014neural}. 

% The two generative models have their own parameters and can be learned joinly by maximizing:
% \begin{equation}
% \label{eq:marginal-sum}
% \gL(\thetax, \thetay) = \sE_{\x\sim \pdx, \y\sim \pdy}[\log p(\x; \thetax) + \log p(\y; \thetay)].
% \end{equation}

\subsection{Learning}
\label{sec:learning}
\begin{figure}[!t]
\centering
     \includegraphics[scale=0.13]{figure/inference.png}
     \caption{Depiction of amortized variational approximation. Distributions $q(\bar y | x)$ and $q(\bar x | y)$ represent inference networks that approximate the model's true posterior. Critically, parameters are shared between the generative model and inference networks to tie the learning problems for both domains.}
    \label{fig:inference}
    \vspace{-10pt}
\end{figure}
Ideally, learning should directly optimize the log data likelihood, which is the marginal of our model shown in Eq.~\ref{eq:marginal}. However, due to our model's neural parameterization which does not factorize, computing the data likelihood cannot be accomplished using dynamic programming as can be done with simpler models like the HMM. To overcome the intractability of computing the true data likelihood, we adopt amortized variational inference~\citep{kingma2013auto} in order to derive a surrogate objective for learning, the evidence lower bound (ELBO) on log marginal likelihood\footnote{Note that in practice, we add a weight $\lambda$ (the same to both domains) to the KL term in ELBO since the regularization strength from the pretrained language model varies depending on the datasets, training data size, or language model structures. Such reweighting is proven necessary in many previous work that is trained with ELBO~\citep{bowman2016generating,miao2016language,yin2018structvae}.} :
{\small
\begin{equation}
\label{eq:elbo}
\begin{split}
&\log p(\xc, \yc; \thetaxy, \thetayx) \\
&\geq \gL_{\text{ELBO}}(\xc, \yc; \thetaxy, \thetayx, \phixy, \phiyx) \\
&= \sum\nolimits_i \Big[ \sE_{q(\by | \x^{(i)}; \phiyx)}[\log p(\x^{(i)}|\by; \thetaxy)] - \KL\big(q(\by | \x^{(i)} ; \phiyx) || \ply \big) \Big] \\
&+\ \sum\nolimits_j \underbrace{\Big[ \sE_{q(\bx | \y^{(j)}; \phixy)}[\log p(\y^{(j)}|\bx; \thetayx)]}_{\textrm{Reconstruction likelihood}} - \underbrace{\KL\big(q(\bx | \y^{(j)}; \phixy) || \plx\big) \Big]}_{\textrm{KL regularizer}} 
\end{split}
\end{equation}}
% \begin{equation}
% \label{eq:elbo}
% \begin{split}
% &\log p(\x, \y; \thetaxy, \thetayx) \\ 
% &\geq \gL_{\text{ELBO}}(\x, \y; \thetaxy, \thetayx, \phixy, \phiyx) \\
% &=\sE_{q_{\phiyx}(\by | \x)}[\log p(\x|\by; \thetaxy)] - \KL(q_{\phiyx}(\by | \x) || \ply) \\
% &\quad +\underbrace{\sE_{q_{\phixy}(\bx | \y)}[\log p(\y|\bx; \thetayx)]}_{\textrm{reconstruction likelihood}} - \underbrace{\KL(q_{\phixy}(\bx | \y) || \plx)}_{\textrm{KL regularizer}}
% \end{split}
% \end{equation}
The surrogate objective introduces $\qyx$ and $\qxy$, which represent two separate inference network distributions that approximate the model's true posteriors, $\ppyx$ and $\ppxy$, respectively. Learning operates by jointly optimizing the lower bound over both variational and model parameters. Once trained, the variational posterior distributions can be used directly for sequence transduction. The KL terms in Eq.~\ref{eq:elbo}, that appear naturally in the ELBO objective, can be intuitively viewed as regularizers that use the language model priors to bias the induced sentences towards the desired domains. Amortized variational techniques have been most commonly applied to continuous latent variables, as in the case of the variational autoencoder (VAE) \citep{kingma2013auto}. Here, we use this approach for inference over discrete sequences, which has been shown to be effective in related work on a semi-supervised task \citep{miao2016language}.
% Note that we add a weight $\lambda$ to the KL term since the regularization strength from the pretrained language model varies depending on the datasets, training data size, or language model structures. 
% $\lambda$ is a tunable hyperparameter in our approach. 
% The inference network is also parameterized as an encoder-decoder structure. \tberg{Move description of inference network architecture to "Parameter Sharing" Section and spend more time describing why we want the same architecture as for the decoder.} Symmetrically, there is another inference network conditioned on $\y$ to approximate $p_{\thetay}(\x | \y)$, and we train the whole model to maximize a lower bound of Eq.~\ref{eq:marginal-sum}:
\vspace{-5pt}
\paragraph{Inference Network and Parameter Sharing: }Note that the approximate posterior on one domain aims to learn the \textit{reverse} transduction distribution, which is exactly the goal of the generative distribution in the opposite domain. For example, the inference network $\qyx$ and the generative distribution $p(\y|\bx^{(i)}; \thetayx)$ both aim to learn to transform from $\xc$ to $\yc$. 
% thus we think there should be only one set of parameter for each direction of transduction. 
Therefore, we use the same architecture for each inference network as used in the transduction models, and tie the parameters of them: $\phixy=\thetaxy, \phiyx=\thetayx$.
This means we learn only two encoder-decoders overall -- which are parameterized by $\thetaxy$ and $\thetayx$ respectively -- to represent two directions of transduction. In addition to reducing number of learnable parameters, this parameter tying couples the learning problems for both domains and allows us to jointly learn from the full data. Moreover, inspired by recent work that builds a universal Seq2Seq model to translates between different language pairs~\citep{johnson2017google}, we introduce further parameter tying between the two directions of transduction: the same encoder is employed for both $\x$ and $\y$, and a domain embedding $c$ is provided to the same decoder to specify the transfer direction, as shown in Figure~\ref{fig:inference}. Ablation analysis in Section~\ref{sec:exp-decipher} suggests that parameter sharing is important to achieve good performance.
% Together, this means we only need to optimize over $\vtheta=\phixy=\thetaxy=\phiyx=\thetayx$ in Eq.~\ref{eq:elbo}.
% \begin{equation} 
% \label{eq:full}
% \begin{split}
% \gL_{\text{ELBO}}(\vtheta) &= \sE_{\x \sim \pdx}\big[\sE_{q_{\vtheta}(\y | \x)}[\log p(\x|\y; \vtheta)] - \KL(q_{\vtheta}(\y | \x) || \ply)\big] \\
% &+ \sE_{\y\sim \pdy}\big[\sE_{q_{\vtheta}(\x | \y)}[\log p(\y|\x; \vtheta)] - \KL(q_{\vtheta}(\x | \y) || \plx)\big]
% \end{split}
% \end{equation}

\vspace{-5pt}
\paragraph{Approximating Gradients of ELBO: } The reconstruction terms and the KL terms in Eq.~\ref{eq:elbo} still involve intractable expectations due to the marginalization of the latent sequence, thus we need to approximate their gradients. We can approximate the expectations by sampling latent sequences, but gradients are difficult to back-propagate directly through discrete samples. Gumbel-softmax~\citep{jang2016categorical} and REINFORCE~\citep{sutton2000policy} are often used as stochastic gradient estimators in the discrete case. Since the latent text variables have an extremely large domain, we find that REINFORCE-based gradient estimates result in high variance. Thus, we use the Gumbel-softmax straight-through estimator to backpropagate gradients from the KL terms. However, we find that approximating gradients of the reconstruction loss is much more challenging -- both the Gumbel-softmax estimator and REINFORCE are unable to outperform a simple stop-gradient baseline, which confirms a similar observation in previous work on unsupervised machine translation~\citep{lample2018phrase}. 
Therefore, we simply stop computing the gradients for the inference network that would result from the reconstruction term, and perform greedy sampling of the latent sequences during training.\footnote{We use one sample to approximate the expectations.} We consider this to be the best empirical compromise at the moment. 
\vspace{-5pt}
\paragraph{Initialization. }Good initialization is often necessary for successful optimization of unsupervised learning objectives. In preliminary experiments, we find that the encoder-decoder structure has difficulty generating realistic sentences during the initial stages of training, which usually results in a disastrous local optimum. This is mainly because the encoder-decoder is initialized randomly and there is no direct training signal to specify the desired latent sequence in the unsupervised setting. Therefore, we apply a self-reconstruction loss $\gL_{\text{rec}}$ at the initial epochs of training. We denote the output the encoder as $e(\cdot)$ and the decoder distribution as $p_{\text{dec}}$, then
\begin{equation}
\label{eq:self-rec}
\gL_{\text{rec}} = -\alpha \cdot \sum\nolimits_i[p_{\text{dec}}(e(\x^{(i}), \cx)] - \alpha \cdot \sum\nolimits_j[p_{\text{dec}}(e(\y^{(j}), \cy)],
\end{equation}
$\alpha$ decays from 1.0 to 0.0 linearly in the first $k$ epochs. $k$ is a tunable parameter and usually less than 3 in all our experiments. 
% [comparison after introducing learning] Traditional sequence to sequence generative models (e.g.\ the noisy channel model) for unsupervised sequence transduction~\citep{knight2006unsupervised} follows the well-known noisy-channel framework, our model makes few assumptions about the transduction distribution and can 
